Mix-CPT: A Domain Adaptation Framework via Decoupling Knowledge Learning and Format Alignment

Adapting general large language models (LLMs) to specialized domains presents great challenges due to varied data distributions. This adaptation typically requires continual pre-training on massive domain-specific corpora to facilitate knowledge memorization, followed by training to apply this knowledge following human instructions and preferences. However, this method may result in inefficient knowledge memorization due to a lack of awareness of knowledge utilization and imposes substantial demands on LLMs to simultaneously learn knowledge utilization and format alignment with limited training samples. To facilitate the domain adaptation of LLM, we revise this process and propose a new domain adaptation framework including domain knowledge learning and general format alignment, called Mix-CPT. Specifically, we first conduct a knowledge mixture continual pre-training that concurrently focuses on knowledge memorization and utilization, allowing for mutual reinforcement. To avoid catastrophic forgetting during the continual pre-training process, we further incorporate a logit swap self-distillation constraint. Subsequently, leveraging the knowledge and capabilities acquired during continual pre-training, we efficiently perform instruction tuning and alignment with a few general training samples to achieve format alignment. Extensive experiments demonstrate that our proposed Mix-CPT framework can simultaneously improve the task-solving capabilities of LLMs on the target and general domains compared to the traditional adaptation methods.

==> sec-app.tex <==
%\section{Appendix}
\label{sec-app}

\begin{table}[htbp]
	\centering
	\small
	\caption{Analysis of MetaQA datasets.}
    \label{tab:dataset_statistics}
    \begin{tabular}{c|c|c|c}
    \hline
    Dataset  & \# of templates & \tabincell{c}{average \# of training \\ cases per template} & \tabincell{c}{\# of used relations for \\ question construction} \\
    \hline
    MetaQA-1 & 161             & 597                                       & 9                                              \\
    MetaQA-2 & 210             & 567                                       & 9                                              \\
    MetaQA-3 & 150             & 761                                       & 9                                              \\
    \hline
\end{tabular}
\end{table}

\section{Datasets}
\label{app:datasets}

We adopt three widely-used multi-hop KGQA datasets in this work:

$\bullet$ \textbf{MetaQA}~\citep{metaqa-aaai-18} contains more than 400k questions in the domain of movie and the answer entities are up to 3 hops away from the topic entities. %We use the MetaQA-1hop, MetaQA-2hop, and MetaQA-3hop datasets split by the hop number.
According to the number of hops, this dataset is split into three sub-datasets, \ie MetaQA-1hop, MetaQA-2hop, and MetaQA-3hop.

$\bullet$ \textbf{WebQuestionsSP (WebQSP)}~\citep{webqsp-acl-15} contains 4,737 questions and the answer entities require up to 2-hop reasoning on the KG Freebase~\citep{freebase-sigmod-08}. 
We use the same train/valid/test splits as GraftNet~\citep{sun-emnlp-18}.

$\bullet$ \textbf{Complex WebQuestions 1.1 (CWQ)}~\citep{cwq-naacl-18} is constructed based on WebQSP by extending the question entities or adding constraints to answers. These questions require up to 4-hop reasoning on the KG Freebase~\citep{freebase-sigmod-08}.

Existing work has demonstrated that the training data for MetaQA is \emph{more than sufficient}~\citep{shi-emnlp-21, he-wsdm-21}, hence all the comparison methods in our experiments can achieve very high performance.
We conduct further analysis of the three MetaQA datasets about the number of templates, the average number of training cases per template, and the number of relations used for constructing questions, and show them in Table~\ref{tab:dataset_statistics}.
In summary, more training cases and simpler questions make the MetaQA easier to be solved.


\section{Baselines}
\label{app:baselines}
We consider the following baseline methods for performance comparison:
%\begin{itemize}

    $\bullet$ \textbf{KV-Mem}~\citep{miller-emnlp-16} maintains a key-value memory table to store KG facts, and conducts multi-hop reasoning by performing iterative read operations on the memory.

	$\bullet$ \textbf{GraftNet}~\citep{sun-emnlp-18} first retrieves the question-relevant subgraph and text sentences from the KG and Wikipedia respectively with a heuristic method. Then it adopts a graph neural network to perform multi-hop reasoning on a heterogeneous graph built upon the subgraph and text sentences.
	
	$\bullet$ \textbf{PullNet}~\citep{sun-emnlp-19} trains a graph retrieval model composed of a LSTM and a graph neural network instead of the heuristic way in GraftNet for the retrieval task, and then conducts multi-hop reasoning with GraftNet.
% 	$\bullet$ \textbf{PullNet}~\citep{sun-emnlp-19} trains a graph retrieval model instead of the heuristic way in GraftNet for the retrieval task, and then conducts multi-hop reasoning with GraftNet.
	
% 	$\bullet$ \textbf{SRN}~\cite{qiu-wsdm-20} directly addresses the multi-hop reasoning by extending relation paths on the KG in an RL setting.
	
	$\bullet$ \textbf{EmbedKGQA}~\citep{saxena-acl-20} reformulates the multi-hop reasoning of GraftNet as a link prediction task by matching pre-trained entity embeddings with question representations from a PLM.
	
	$\bullet$ \textbf{NSM}~\citep{he-wsdm-21} first conducts retrieval following GraftNet and then adapt the neural state machine~\citep{nsm-nips-19} used in visual reasoning for multi-hop reasoning on the KG.
	
	$\bullet$ \textbf{TransferNet}~\citep{shi-emnlp-21} first conducts retrieval following GraftNet and then performs the multi-hop reasoning on a KG or a text-formed relation graph in a transparent framework. The reasoning model consists of a PLM for question encoding and a graph neural network for updating the relevance scores between entities and the question.
	
	$\bullet$ \textbf{SR+NSM}~\citep{zhang-acl-22} first learns a PLM-based relation path retriever to conduct effectively retrieval and then leverages NSM reasoner to perform multi-hop reasoning.
	
	$\bullet$ \textbf{SR+NSM+E2E}~\citep{zhang-acl-22} further fine-tunes the SR\text{+}NSM by an end-to-end way.% after pre-training the retriever.  
	
%\end{itemize}

\begin{figure}[t]
	\centering
	\subfigure[]{
		\centering
		\includegraphics[width=0.22\textwidth]{resource/step_hits1_webqsp.pdf}
		\label{fig:pretrain_steps}
	}
	\subfigure[]{
		\centering
		\includegraphics[width=0.22\textwidth]{resource/hd_hits1_webqsp.pdf}
		\label{fig:dimension}
	}
	\subfigure[]{
		\centering
		\includegraphics[width=0.215\textwidth]{resource/topk_acr_webqsp.pdf}
		\label{fig:topk}
	}
% 	\subfigure[]{
% 		\centering
% 		\includegraphics[width=0.215\textwidth]{resource/epoch_hits1_webqsp.pdf}
% 		\label{fig:epoch}
% 	}
	\centering
	\caption{(a) the performance on WebQSP of varying pre-training steps, (b) hidden dimensions, and (c) the number of retrieved nodes $K$.}
	\label{fig:comprehension-few-shot}
\end{figure}

\section{Knowledge Graph Preprocessing Details}
\label{app:implementation}
We preprocess the full Freebase following existing work~\citep{sun-emnlp-18, he-wsdm-21}. 
For MetaQA, we directly use the subset of WikiMovies provided by the datasets, and the size is about 134,741.
For WebQSP and CWQ datasets, we set the max hops of retrieval and reasoning as two and four for the WebQSP and CWQ, respectively. 
Based on the topic entities labeled in original datasets, we reserve the neighborhood subgraph consisting of entities within the four hops of the topic entities for each sample. After such simple preprocessing, the size of KG we used is 147,748,092 for WebQSP and 202,358,414 for CWQ. 
Based on the preprocessed KG, we conduct the retrieval and reasoning using our proposed approach. 
%As we can see, such a large scale increases the task difficulty and enforces a convincing performance comparison. 


\section{Implementation Details.}
During pre-training, we collect question-relation pairs based on the shortest relation paths between topic entities and answer entities, and then use these pairs to pre-train the RoBERTa~\citep{roberta-arxiv-19} model with the contrastive learning objective. 
We set the temperature $\tau$ as 0.05, and select the best model by evaluating \textit{Hits@1} on the validation set.
For retrieval and reasoning, we initialize the PLM module of our UniKGQA model with the contrastive learning pre-trained RoBERTa, and set the hidden size of other linear layers as 768.
% The learning rate is tuned amongst {0.01, 0.005, 0.001, 0.0005, 0.0001}.
We optimize parameters with the AdamW optimizer, where the learning rate is 0.00001 for the PLM module, and 0.0005 for other parameters.
The batch size is set to 40. 
%, which already performs well and is not tuned further.
The reasoning step is set to 4 for CWQ dataset, and 3 for other datasets.
We preprocess the KGs for each datasets following existing work~\citep{sun-emnlp-18, he-wsdm-21}.
%We present the detailed description of the KG preprocessing in Appendix~\ref{app:implementation}.
% Specifically, with the topic entities labeled in original datasets, we extract the neighborhood graph within the max hops~(\ie reasoning steps) of the topic entities for each sample as the initial subgraph. 
% By aggregating all the initial subgraphs of each sample, we can get the preprocessed KGs.
% After the preprocessing, we conduct the retrieval and reasoning with our proposed approach. 

\section{One-shot experiment for MetaQA}
\label{app:one-shot}
%Due to the training data for MetaQA is more than sufficient, we further conduct an one-shot experiment following NSM~\cite{he-wsdm-21}. 
%We randomly sample a single training case for every question template from the original training set, which forms a one-shot training dataset. 
%The number of training samples for MetaQA-1, MetaQA-2, and MetaQA-3 are 161, 210, and 150, respectively. 
%We evaluate the performance of our approach and some strong baselines (i.e., TrasnferNet and NSM) trained with this new training dataset. 
%As shown in Table~\ref{tab:one-shot}, our method can consistently obtain improvement on all three subsets.

\begin{table}[htbp]
	\centering
	\small
	\caption{One-shot experiment results on MetaQA (Hits@1 in percent).}
    \label{tab:one-shot}
    \begin{tabular}{c|c|c|c}
    \hline
    Model  & MetaQA-1 & MetaQA-2  & MetaQA-3 \\
    \hline
    NSM & 94.8 & 97.0 & 91.0 \\
    TransferNet & 96.5 & 97.5 & 90.1 \\
    UniKGQA & 97.1 & 98.2 & 92.6 \\
    \hline
\end{tabular}
\end{table}

Since the samples in MetaQA are more than sufficient, all the comparison methods in our experiments have achieved very high performance. For example, our method and previous work (\eg TransferNet and NSM) have achieved more than 98\% Hits@1 on MetaQA, which shows that this dataset's performance may have been saturated. 
To examine this assumption, we consider conducting few-shot experiments to verify the performance of different methods. Specially, we follow the NSM paper~\citep{he-wsdm-21} that conducts the one-shot experiment. We randomly sample just one training case for each question template from the original training set, to form a one-shot training dataset. In this way, the numbers of training samples for MetaQA-1, MetaQA-2, and MetaQA-3 are 161, 210, and 150, respectively. We evaluate the performance of our approach and some strong baselines (\ie TrasnferNet and NSM) trained with this new training dataset. As shown in Table~\ref{tab:one-shot}, our method can consistently outperform these baselines in all three subsets. 


\section{Ablation Study of our Unified Model Architecture}

\begin{table}[htbp]
	\centering
	\small
	\caption{Ablation study by combining our UniKGQA with other models.}
    \label{tab:ablation_unified}
    \begin{tabular}{l|c|c}
    \hline
    Models  & WebQSP (Hits@1) & CWQ (Hits@1) \\
    \hline
    PPR+NSM & 68.7 & 47.6 \\
    SR+NSM & 68.9 & 50.2 \\
    SR+UniKGQA & 70.5 & 48.0 \\
    UniKGQA+NSM   & 69.1 & 49.2\\
    UniKGQA+UniKGQA & 75.1 & 50.7\\
    \hline
\end{tabular}
\end{table}

The unified model architecture is the key of our approach. 
Once the unified model architecture is removed, it would be hard to share the question-relation matching capability enhanced by pre-training in retrieval and reasoning stages, and also hard to transfer the relevance information for multi-hop KGQA learned in the retrieval stage to the reasoning stage. 
To verify it, we conduct an extra ablation study to explore the effect of only adopting the unified model architecture as the reasoning model or the retrieval model. We select the existing strong retrieval model (\ie SR) and reasoning model (\ie NSM), and compare the performance when integrated with our UniKGQA.
As we can see in Table~\ref{tab:ablation_unified}, all the variants underperform our UniKGQA. It indicates that the unified model used in the retrieval and reasoning stages simultaneously is indeed the key reason for improvement.


\section{Analysis of the Pre-training Strategy}

\begin{table}[htbp]
	\centering
	\small
	\caption{Results of variants with or without pre-training strategy (Pre) and updating the PLM (QU).}
    \label{tab:ablation_techniques}
    \begin{tabular}{l|c|c}
    \hline
    Models  & WebQSP (Hits@1) & CWQ (Hits@1) \\
    \hline
    UniKGQA & 75.1 & 50.7 \\
    \hline
    w QU & 77.0 & 50.9 \\
    w/o Pre, w QU & 75.4 & 49.2\\
    w/o Pre & 67.3 & 48.1 \\
    \hline
\end{tabular}
\end{table}

We conduct the analysis experiments to investigate how the pre-training strategy (Pre) affects the performance with or without updating the PLM (QU). We show the results in Table~\ref{tab:ablation_techniques}. Once removing the pre-training strategy, the model performance would drop 10.4\% (2.1\%) in WebQSP and 5.1\% (3.3\%) in CWQ when fixing (not fixing) the PLM. It indicates that the pre-training strategy is an important component of our approach. After pre-training, the PLM can be fixed for more efficient parameters optimization during fine-tuning.

\section{Parameter Sensitivity Analysis} 
\label{app:sensitivity}

\paratitle{Pre-training Steps} 
Although the pre-training strategy has shown effective in our approach, too many pre-training steps will be time-consuming and costly.
Here, we investigate the performance with respect to varying pre-training steps.
As shown in Figure~\ref{fig:pretrain_steps}, we can see that our method can reach the best performance with only few pre-training steps (\ie 2800) compared with the best baseline TransferNet.
It shows that our approach does not require too many steps for pre-training.
Instead, we can see that too many pre-training steps will hurt the model performance. The reason may be that the PLM has overfit into the contrastive learning objective.

\paratitle{Parameter Tuning.} In our approach, we have two hyper-parameters required to tune:
(1) the hidden size of linear layers $d$ and (2) the number of retrieved nodes $K$.
Here, we tune the $d$ amongst \{64, 128, 256, 512, 768, 1024\} and $K$ amongst \{1, 5, 10, 15, 20\}.
We show the results in Figure~\ref{fig:dimension} and Figure~\ref{fig:topk} compared with the best results for the reasoning stage and the retrieval stage.
Since $K$ is a consistent hyper-parameter in the UniKGQA and SR, we also describe the various results of SR with different $K$ to give a fair comparison.
First, we can see that our method is robust to different hidden sizes, as the performance is consistently nearby 77.0.
As the PLM adopts 768 as the embedding size, we can see 768 is also slightly better than other numbers.
Besides, we can see that with the increase of $K$, the answer coverage rate also improves consistently.
However, when $K$ increases to 15 or even 20, the performance gain becomes relatively small. 
It means that the retrieved subgraphs are likely saturated, and further increasing $K$ could only bring marginal improvement.

==> sec-pre.tex <==
\section{Preliminary}
In this section, we introduce the notations that will be used throughout the paper and then formally define the multi-hop KGQA task.

\paratitle{Knowledge Graph~(KG).} A knowledge graph typically consists of a set of triples, denoted by $\mathcal{G} = \{\langle e,r,e' \rangle| e,e' \in \mathcal{E}, r \in \mathcal{R}\}$, where $\mathcal{E}$ and $\mathcal{R}$ denote the entity set and relation set, respectively. 
A triple $\langle e,r,e' \rangle$ describes the fact that a relation $r$ exists between head entity $e$ and tail entity $e'$.
Furthermore,  we denote the set of neighborhood triples that an entity $e$ belongs to by $\mathcal{N}_e = \{\langle e, r, e' \rangle \in \mathcal{G} \} \cup \{\langle e', r, e \rangle \in \mathcal{G} \}$.
Let $r^{-1}$ denote the inverse relation of $r$, and we can represent 
a triple $\langle e, r, e' \rangle$ by its inverse triple $\langle e', r^{-1}, e \rangle$. In this way, we can simplify the definition of  the neighborhood triples for an entity $e$ as $\mathcal{N}_e=\{\langle e', r, e \rangle \in \mathcal{G} \}$.
We further use $\bm{E} \in \mathbb{R}^{d \times |\mathcal{E}|}$ and $\bm{R} \in \mathbb{R}^{d \times |\mathcal{R}|}$ to denote the embedding matrices for entities and relations in KG, respectively.




%$= \{\langle e,r,e'_{a} \rangle| \langle e,r,?\rangle \subset \mathcal{G}\}$.

%Given a original subgraph 
%$\mathcal{G}_a = \{\langle e,r,e'_{a} \rangle| \langle e,r,?\rangle \subset \mathcal{G}\}$

%Specifically, starting from the topic entities, the abstract subgraph merges all tail entities $\{e'\}$ affiliated with the same relation $r$, denoted by $\mathcal{G}_a = \{\langle e,r,e'_{a} \rangle| \langle e,r,?\rangle \subset \mathcal{G}\}$

\paratitle{Multi-hop Knowledge Graph Question Answering~(Multi-hop KGQA).} 
%We focus on multi-hop factoid question answering over a knowledge graph. 
Given a natural language question $q$ and a KG $\mathcal{G}$, the task of KGQA aims to find answer entitie(s) to the question over the KG, denoted by the answer set $\mathcal{A}_q \in \mathcal{E}$.
Following previous work~\citep{sun-emnlp-18, sun-emnlp-19}, we assume that the entities mentioned in the question (\eg ``The Jeff Probst Show'' in Figure~\ref{fig:model}(a) are marked and linked with entities on KG,  namely \emph{topic entities}, denoted as $\mathcal{T}_q \subset \mathcal{E}$.
In this work, we focus on solving the \emph{multi-hop KGQA} task where the answer entities are multiple hops away from the topic entities over the KG.
Considering the trade-off between efficiency and accuracy, we follow existing work~\citep{sun-emnlp-18, sun-emnlp-19} that solves this task using a \emph{retrieval}-then-\emph{reasoning} framework.  In the two-stage framework, given a question $q$ and topic entities $\mathcal{T}_q$, the retrieval model aims to retrieve a small subgraph $\mathcal{G}_q$ from the large-scale input KG $\mathcal{G}$, while the reasoning model searches answer entities $\mathcal{A}_q$ by reasoning over the retrieved subgraph $\mathcal{G}_q$. 


\paratitle{Abstract Subgraph.} Based on KGs, we further introduce the concept of \emph{abstract graph}, which is derived based on the reduction from an original subgraph. 
Specifically, given a subgraph related to question $q$, denoted as $\mathcal{G}_q \subset \mathcal{G}$, 
we merge the tail entities from the triples with the same \emph{prefix} (\ie the same head entity and relation: $\langle e,r, ? \rangle$), and then generate a corresponding abstract node $\widetilde{e}$ to represent the set of tail entities, so we have $\tilde{e}=\{e' | \langle e,r,e' \rangle\in \mathcal{G}\}$. 
Similarly, we can also perform the same operations on the head entities. 
To unify the notations, we transform an original node that can't be merged into an abstract node by creating a set including the node itself. 
In this way, the corresponding abstract subgraph $\mathcal{G}_q$ can be denoted as: $\widetilde{\mathcal{G}}_q = \{\langle \tilde{e},r,\tilde{e}' \rangle | \exists e \in \tilde{e}, \exists  e' \in \tilde{e}', \langle e,r,e' \rangle \in \mathcal{G}_q\}$, where each node $\tilde{e}$ is an abstract node representing a set of original nodes (one or multiple). We present an illustrative example of the original subgraph and its abstract subgraph in Figure~\ref{fig:model}(a) and Figure~\ref{fig:model}(b).

\ignore{
\paratitle{Retrieval-then-Reasoning.} Considering the efficiency and accuracy, we follow existing work~\citep{sun-emnlp-18, sun-emnlp-19} that solves this task using a two-stage \emph{retrieval}-then-\emph{reasoning} framework.  In the two-stage framework, given a question $q$ and topic entities $\mathcal{T}_q$, the retrieval part aims to retrieve a very small subgraph $\mathcal{G}_r$ from the large-scale input KG $\mathcal{G}$, while the reasoning part searches answer entities $\mathcal{A}_q$ by performing reasoning on the small subgraph $\mathcal{G}_q$. Considering the huge scale difference of the input search space for the two parts (\ie $\mathcal{G}$ and $\mathcal{G}_q$), we introduce an \emph{abstract subgraph} to reduce the size of the large-scale KG. Specifically, starting from the topic entities, the abstract subgraph merges all tail entities $\{e'\}$ affiliated with the same relation $r$, denoted by $\mathcal{G}_a = \{\langle e,r,e'_{a} \rangle| \langle e,r,?\rangle \subset \mathcal{G}\}$. In this way, the number of neighbourhood triples for each entity in KG can be extremely reduced to the number of relation types. We show an abstract subgraph example in the middle of Fig~\ref{fig:model}. Therefore, we can unify the learning objective of the retrieval and reasoning parts as: given a question $q$ and a very small subgraph $\mathcal{G}_s$ (\ie $\mathcal{G}_s$ equals to the abstracted KG subgraph $\mathcal{G}_a$ in the retrieval stage or the retrieved subgraph $\mathcal{G}_q$ in the reasoning stage), the model should predict the match scores $\bm{s}$ of each candidate node in the $\mathcal{G}_s$ according to the question semantics.
}



